Generalized Few-Shot Semantic Segmentation: All You Need is Fine-Tuning

Generalized few-shot semantic segmentation was introduced to move beyond only evaluating few-shot segmentation models on novel classes to include testing their ability to remember base classes. While the current state-of-the-art approach is based on meta-learning, it performs poorly and saturates in learning after observing only a few shots. We propose the first fine-tuning solution, and demonstrate that it addresses the saturation problem while achieving state-of-the-art results on two datasets, PASCAL-5i and COCO-20i. We also show that it outperforms existing methods, whether fine-tuning multiple final layers or only the final layer. Finally, we present a triplet loss regularization that shows how to redistribute the balance of performance between novel and base categories so that there is a smaller gap between them.

==> discussion.tex <==
\section{Discussion}
In this work we showed that fine-tuning can be a better alternative to meta-learning for generalized few-shot semantic segmentation, especially as the number of available shots increase. However, another interesting observation is that fine-tuning only the last layer in our network leads to worse results than fine-tuning all layers after the backbone. In contrast, Wang et al.~\cite{wang2020frustratingly} reports that fine-tuning only the last layer leads to best results and we confirm in the supplementary materials that fine-tuning all layers after the backbone results in degraded performance. A possible explanation for this is that semantic segmentation produces denser outputs than object detection, but an interesting future work could examine why the features from each respective task do not generalize to novel classes in the same way.

%% Thank Samreen
